The TeV gamma-ray luminosity of the Milky-Way and the contribution of H.E.S.S. unresolved sources to VHE diffuse emission

H.E.S.S. has recently completed a systematic survey of the Galactic plane in the TeV energy domain. We analyze the flux, latitude and longitude distributions of $\gamma-$ray sources observed by H.E.S.S. in order to infer the properties of Galactic TeV source population. We show that the total Milky-Way luminosity in the 1-100 TeV energy range is $L_{\rm MW} = 1.7^{+0.5}_{-0.4}\times 10^{37} {\rm ergs}\,{\rm sec}^{-1}$. Evaluating the cumulative flux expected at Earth by the considered population, we show that H.E.S.S. unresolved sources provide a relevant contribution to the diffuse Galactic emission. Finally, in the hypothesis that the majority of bright sources detected by H.E.S.S. are powered by pulsar activity, like e.g. Pulsar Wind Nebulae or TeV halos, we estimate the main properties of the pulsar population.

==> preamble.tex <==
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry} 
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage{lipsum}
\usepackage{csquotes}

==> sections/section03bis.tex <==
\section{Pulsar Wind Nebulae} \label{sec:fading}
The above description can be applied to potential TeV sources in the Galaxy, such as Pulsar Wind Nebulae or TeV Halos, which are connected  with the explosion core-collapse SN and the formation of a pulsar. 
%
The birth rate of these objects can be assumed proportional to that of SN explosions in our Galaxy, i.e. $R_{\rm SN} = 0.019\,{\rm yr}^{-1}$ as recently measured by \cite{Linden}. We thus write $R=\varepsilon \, R_{\rm SN}$ assuming $\varepsilon = 1$ for simplicity, unless otherwise specified. 


If the TeV-emission is powered by pulsar activity it is reasonable to assume that TeV-luminosity is proportional to the pulsar spindown power that can be expressed as:
\begin{equation}
\Dot{E} = \Dot{E}_0 \left(1+\frac{t}{\tau_{\rm sd}}\right)^{-2}
\end{equation}
%
with:
\begin{eqnarray}
\nonumber
\Dot{E}_0 &=&\frac{8\pi^4 B_0^2 R^6}{3 c^3 P_0^4}\\
\tau_{\rm sd} &=& \frac{3 I c^3 P_0^2}{4\pi^2B_0^2 R^6}
\end{eqnarray}
where $P_0$ and $B_0$ are the initial spin period and magnetic fields \cite{Shapiro} while $M=1.4\,M_{\odot}$ and $R= 12 \,{\rm km}$ \cite{Lattimer:2006xb}. 
%
This implies that the fading timescale is determined by the pulsar spindown time scale, i.e. $\tau = \tau_{\rm sd}$, the exponent in Eq.\eqref{lum} is $\gamma=2$ so that the luminosity distribution scales as $Y(L)\propto L^{-1.5}$. The maximal luminosity is a fraction of the initial spindown power, i.e. $L_{\rm max}\simeq \eta \Dot{E}_0$, with $\eta \simeq 0.1$ was suggested e.g. by \cite{Sudoh:2019lav,Manconi:2020ipm} in connection with total $e^{\pm}$ luminosity observed by AMS-02. 
